Stochastic Optimization with Bandit Sampling

Many stochastic optimization algorithms work by estimating the gradient of the cost function on the fly by sampling datapoints uniformly at random from a training set. However, the estimator might have a large variance, which inadvertently slows down the convergence rate of the algorithms. One way to reduce this variance is to sample the datapoints from a carefully selected non-uniform distribution. In this work, we propose a novel non-uniform sampling approach that uses the multi-armed bandit framework. Theoretically, we show that our algorithm asymptotically approximates the optimal variance within a factor of 3. Empirically, we show that using this datapoint-selection technique results in a significant reduction in the convergence time and variance of several stochastic optimization algorithms such as SGD, SVRG and SAGA. This approach for sampling datapoints is general, and can be used in conjunction with any algorithm that uses an unbiased gradient estimation -- we expect it to have broad applicability beyond the specific examples explored in this work.

==> sup.tex <==

\begin{proof}
	The proof is similar to the most of multiplicative-weight update algorithms proof. In fact, we follow the proof of Theorem 3.1 in \cite{BC2012} with the additional bookkeeping that the in our algorithm each probabilities is bounded from below. 
	Let $l_i^t = -\frac{a_i^t}{(P^t_i)^2}$ be the loss of point $i$ and its negative $r_i(t) = \frac{a_i^t}{(P^t_i)^2}$ be the reward of point $i$. Note that $\hat{l}^t_i  =l_i^t*1_{\{I_t=i\}}/P^t_i$ is an unbiased estimator of $l_i^t$. First, we write $\hat{l}^t_i$ as follows
		\begin{equation}\label{eq:eq1}
		\begin{aligned}
		&\mathbb{E}_{I_t\sim P^t}\mathbb{E}_{j\sim P^t}[\hat{l}_j^t] = \sum_{i=1}^{n}P^t_il^t_i
		\\&\leq \frac{1}{\delta}\left(\ln \mathbb{E}_{I_t\sim P^t}\mathbb{E}_{j\sim P^t}\left[\exp\left(-\delta\left(\hat{l}_j^t-\mathbb{E}_{I_t\sim P^t}\mathbb{E}_{j\sim P^t}[\hat{l}_j^t]\right)\right)\right]
		-\ln \mathbb{E}_{I_t\sim P^t}\mathbb{E}_{j\sim P^t}\left[\exp\left(-\delta\hat{l}_j^t\right)\right]\right).
		\end{aligned}
		\end{equation}
	Now we can use the inequalities for $\ln$ to find a bound on the estimator of losses, and by applying expectation we can find the bound on the expected value of losses. Applying the inequalities $\ln x \leq x-1$ and $\exp(-x)-1+x\leq x^2$ to the first term in Equation~\ref{eq:eq1} we have
	\begin{equation}
	\begin{aligned}
	\frac{1}{\delta}\ln \mathbb{E}_{I_t\sim P^t}\mathbb{E}_{j\sim P^t}\left[\exp\left(-\delta(\hat{l}_j^t-\mathbb{E}[\hat{l}_j^t])\right)\right]&\leq
	\mathbb{E}_{I_t\sim P^t}[\frac{\delta}{2} \frac{(l^t_j)^2}{P^t_{I_t}}] =\frac{\delta}{2} \sum_{i=1}^{n} (l_i^t)^2.
	\end{aligned}
	\end{equation}
	We can bound the second term of Equation~\eqref{eq:eq1} as follows
		\begin{equation}\label{eq:eq2}
		\begin{aligned}
		-\frac{1}{\delta} \ln \mathbb{E}_{I_t\sim P^t}\mathbb{E}_{j\sim P^t} &\exp(-\delta \hat{l}_j^t)  \leq
		-\frac{1}{\delta} \mathbb{E}_{I_t\sim P^t} \ln \mathbb{E}_{j\sim P^t} \exp(-\delta \hat{l}_j^t) \\ & =
		-\frac{1}{\delta} \mathbb{E}_{I_t\sim P^t} \ln \sum_{j=1}^{K}P^t_j \exp(-\delta \hat{l}_j^t) \\ &=
		-\frac{1}{\delta} \mathbb{E}_{I_t\sim P^t}\left[ \ln\left( \sum_{j=1}^{K}(1-\eta) \frac{\exp(-\delta \hat{L}_j^t)}{\sum_{c=1}^{K}\exp(-\delta \hat{L}_c^{t-1})}+\frac{\eta}{K}\exp(-\delta\hat{l}_j(t))\right)\right] \\&\leq   
		-\frac{1}{\delta}\mathbb{E}_{I_t\sim P^t}\left( \frac{\eta}{K}\sum_{j=1}^K(-\delta\hat{l}_j^t) +(1-\eta)\left[ \ln\left(\sum_{j=1}^{K}\frac{\exp(-\delta \hat{L}_j^t)}{\sum_{c=1}^{K}\exp(-\delta \hat{L}_c^{t-1})}\right)\right]       \right)     ,                           
		\end{aligned}
		\end{equation} 
		where $\hat{L}_j^t = \sum_{h=1}^{t}\hat{l}_j^h$ and we use Jensen's inequality in the first and last inequality. The second term of right-hand side of above equation is bounded as follows
		\begin{equation}
		\begin{aligned}
		-\frac{(1-\eta)}{\delta}\mathbb{E}_{I_t\sim P^t}\left[ \ln\left(\sum_{j=1}^{K}\frac{\exp(-\delta \hat{L}_j^t)}{\sum_{c=1}^{K}\exp(-\delta \hat{L}_c^{t-1})}\right)\right] &\leq  \frac{(1-\eta)\ln n}{\delta} + \mathbb{E}_{I_t\sim P^t} [\hat{L}^t_k] \\
		& = \frac{(1-\eta)\ln n}{\delta} + L^t_k .		
		\end{aligned}
		\end{equation}
	By substituting these inequalities in Equation~\eqref{eq:eq1} we get,
	\begin{equation} \label{eq:final}
	\sum_{t=1}^{T} \sum_{i=1}^{n} P^t_il^t_i \leq \frac{\delta}{2} \sum_{t=1}^{T}\sum_{i=1}^{n} (l^t_i)^2+\sum_{t=1}^{T}\frac{\eta}{K} \mathbb{E}_{a_t\sim p^\prime_t} \sum_{c=1}^K\hat{l}_c(t)+\frac{\ln K}{\delta}+\mathbb{E}_{a_t\sim p^\prime_t} [\hat{L}_k(T)].
	\end{equation}
\end{proof}


